FathomGPT: A Natural Language Interface for Interactively Exploring Ocean Science Data

We introduce FathomGPT, an open source system for the interactive investigation of ocean science data via a natural language interface. FathomGPT was developed in close collaboration with marine scientists to enable researchers to explore and analyze the FathomNet image database. FathomGPT provides a custom information retrieval pipeline that leverages OpenAI's large language models to enable: the creation of complex queries to retrieve images, taxonomic information, and scientific measurements; mapping common names and morphological features to scientific names; generating interactive charts on demand; and searching by image or specified patterns within an image. In designing FathomGPT, particular emphasis was placed on enhancing the user's experience by facilitating free-form exploration and optimizing response times. We present an architectural overview and implementation details of FathomGPT, along with a series of ablation studies that demonstrate the effectiveness of our approach to name resolution, fine tuning, and prompt modification. We also present usage scenarios of interactive data exploration sessions and document feedback from ocean scientists and machine learning experts.

==> Sections/03_Tasks.tex <==
\section{Tasks} \label{Sec:Tasks}

FathomGPT is built to answer scientific researchers' queries about the FathomNet database. Below are several tasks in which a natural language processing system can assist scientific researchers:
\begin{enumerate}
    \item A Researcher does not have the technical knowledge to get information from the FathomNet database and needs an easy way to access the database in a quick and easy way.
    \item A Researcher needs to label a species found in a new image but is confused about which species it is. He uses an image similarity search on the image he has.
    \item There is a gas leakage in the ocean. A Researcher wants to quickly evaluate what species will get effected at that place. He goes through the visualization to find out what species are found at that location.
    \item A Researcher wants to know the taxonomy of a species.
    \item A Researcher wants to understand how climate change has affected the ecological diversity in an area. To evaluate this, the researcher searches for the species image that were taken at two different times.
    \item A Researcher wants to identify species that utilize similar camouflage techniques. They use the pattern search to find species with similar body patterns.
    \item A Researcher does not remember the name of a species but remembers what they look like. They describe the pattern of the species to find its name and taxonomy.
    \item A Researcher wants to know what are the patterns that frequently show up on species living in an area.
    
\end{enumerate} 

==> Sections/08_Conclusion.tex <==
\section{Conclusion} 




